Observation of a Threshold Enhancement in the $\pi^0\pi^0$ Mass Spectrum in $\psi(3686) \rightarrow \pi^{0}\pi^{0}J/\psi$ Decays

Using a data sample of $(2712.4\pm14.4)\times 10^{6}$ $\psi(3686)$ events collected with the BESIII detector, we report a high-precision study of the $\pi^{0}\pi^{0}$ mass spectrum from $\psi(3686)\rightarrow\pi^{0}\pi^{0}J/\psi$ decays. The enhancement previously observed near the $\pi\pi$ mass threshold in the $\pi^+\pi^-$ channel is confirmed, with a statistical significance exceeding 10$\sigma$. A fit with a Breit-Wigner function yields a mass of $M = 274.3\pm 2.1_{\rm stat.}\pm0.6_{\rm syst.}~{\rm MeV}/c^2$ and a width of $\Gamma = 17.1\pm 1.5_{\rm stat.}\pm0.5_{\rm syst.}~{\rm MeV}$, consistent with those from the $\pi^{+}\pi^{-}$ channel. By including final-state interactions, we analyze the data using both chiral perturbation theory (ChPT) and QCD multipole expansion (QCDME). While the ChPT model describes the higher-mass region above 0.3 GeV/$c^2$ well, it fails to reproduce the significant threshold enhancement. In contrast, the QCDME model, which incorporates the $S$- and $D$-wave admixture structure of $\psi(3686)$, provides a better description of the full $\pi^{0}\pi^{0}$ mass spectrum.

==> acknowledgement_2026-04-17.tex <==
%% Saved at => 2026-04-17
\textbf{Acknowledgement}

The BESIII Collaboration thanks the staff of BEPCII (https://cstr.cn/31109.02.BEPC) and the IHEP computing center for their strong support. This work is supported in part by National Key R\&D Program of China under Contracts Nos. 2023YFA1606000, 2023YFA1606704, 2025YFA1613900; National Natural Science Foundation of China (NSFC) under Contracts Nos. 11635010, 11935015, 11935016, 11935018, 12025502, 12035009, 12035013, 12061131003, 12192260, 12192261, 12192262, 12192263, 12192264, 12192265, 12221005, 12225509, 12235017, 12342502, 12361141819, 12535005; the Chinese Academy of Sciences (CAS) Large-Scale Scientific Facility Program; the Strategic Priority Research Program of Chinese Academy of Sciences under Contract No. XDA0480600; CAS under Contract No. YSBR-101; 100 Talents Program of CAS; The Institute of Nuclear and Particle Physics (INPAC) and Shanghai Key Laboratory for Particle Physics and Cosmology; Agencia Nacional de Investigación y Desarrollo de Chile (ANID), Chile under Contract No. ANID CCTVal CIA250027; ERC under Contract No. 758462; German Research Foundation DFG under Contract No. FOR5327; Istituto Nazionale di Fisica Nucleare, Italy; Knut and Alice Wallenberg Foundation under Contracts Nos. 2021.0174, 2021.0299, 2023.0315; Ministry of Development of Turkey under Contract No. DPT2006K-120470; National Research Foundation of Korea under Contract No. RS-2026-25486791; National Science and Technology fund of Mongolia; Polish National Science Centre under Contract No. 2024/53/B/ST2/00975; STFC (United Kingdom); Swedish Research Council under Contract No. 2019.04595; U. S. Department of Energy under Contract No. DE-FG02-05ER41374

\textbf{Other Fund Information}

To be inserted with an additional sentence into papers that are relevant to the topic of special funding for specific topics. Authors can suggest which to Li Weiguo and/or the physics coordinator.
        Example added sentence: This paper is also supported by the NSFC under Contract Nos. 10805053, 10979059, ....National Natural Science Foundation of China (NSFC), 10805053, PWANational Natural Science Foundation of China (NSFC), 10979059, Lund弦碎裂强子化模型及其通用强子产生器研究National Natural Science Foundation of China (NSFC), 10775075, National Natural Science Foundation of China (NSFC), 10979012, baryonsNational Natural Science Foundation of China (NSFC), 10979038, charmoniumNational Natural Science Foundation of China (NSFC), 10905034, psi(2S)->B BbarNational Natural Science Foundation of China (NSFC), 10975093, D 介子National Natural Science Foundation of China (NSFC), 10979033, psi(2S)->VPNational Natural Science Foundation of China (NSFC), 10979058, hcNational Natural Science Foundation of China (NSFC), 10975143, charmonium rare decays
%% ends here %%

